Bridging the Granularity Gap for Acoustic Modeling

While Transformer has become the de-facto standard for speech, modeling upon the fine-grained frame-level features remains an open challenge of capturing long-distance dependencies and distributing the attention weights. We propose \textit{Progressive Down-Sampling} (PDS) which gradually compresses the acoustic features into coarser-grained units containing more complete semantic information, like text-level representation. In addition, we develop a representation fusion method to alleviate information loss that occurs inevitably during high compression. In this way, we compress the acoustic features into 1/32 of the initial length while achieving better or comparable performances on the speech recognition task. And as a bonus, it yields inference speedups ranging from 1.20$\times$ to 1.47$\times$. By reducing the modeling burden, we also achieve competitive results when training on the more challenging speech translation task.

==> fig/Alignment.tex <==
\definecolor{myyellow}{RGB}{255,215,0}
\definecolor{ugreen}{RGB}{124,205,124}
\definecolor{ublue}{RGB}{39,64,139}
\usetikzlibrary{shapes.geometric,fit,backgrounds,shadows}
\begin{figure}[t!]
\centering
\begin{tikzpicture}
    \tikzstyle{representStyle} = [minimum height=0.7em,rounded corners=1pt,draw,fill=myyellow!15,minimum width=1em]
    \tikzstyle{prob} = [minimum height=0.7em,rounded corners=1pt,fill=ugreen!50,minimum width=1em]

    %%%%%%%%%%%%%%%%%%% 1
    \node[representStyle,minimum width=3em] (rep1) at (0,0) {};
    \node[representStyle,minimum width=2.5em] (rep2) at ([yshift=0.4em,xshift=0em]rep1.north) {};
    \node[](dot1) at ([yshift=0.4em,xshift=0]rep2.north) {.};
    \node[](dot2) at ([yshift=-0.05cm]dot1.north) {.};
    \node[](dot3) at ([yshift=-0.05cm]dot2.north) {.};
    \node[representStyle,minimum width=1em] (rep3) at ([yshift=1.6em,xshift=0em]rep2.north) {};

    %%%%%%%%%%%%%%%%%%% 2
    \node[draw,rounded corners=3pt] (alig) at ([yshift=1.3em,xshift=3.2em]rep1.east) {\small Alignment};

    %%%%%%%%%%%%%%%%%%% 3
    \node[representStyle,minimum width=1em] (rep21) at ([yshift=0em,xshift=7.5em]rep1.east) {};
    \node[representStyle,minimum width=1em] (rep22) at ([yshift=0.4em]rep21.north) {};
    \node[](dot21) at ([yshift=0.4em,xshift=0em]rep22.north) {.};
    \node[](dot22) at ([yshift=-0.05cm]dot21.north) {.};
    \node[](dot23) at ([yshift=-0.05cm]dot22.north) {.};
    \node[representStyle,minimum width=1em] (rep23) at ([yshift=1.6em]rep22.north) {};
    
    \draw[-,line width=1.8pt,ublue] ([xshift=0.6em,yshift=0.9em]rep22.east) -- ([xshift=1.3em,yshift=0.1em]rep22.east);
    \draw[-,line width=1.8pt,ublue] ([xshift=0.6em,yshift=0.1em]rep22.east) -- ([xshift=1.3em,yshift=0.9em]rep22.east);

    \draw[->,line width=1.8pt,ublue] ([xshift=-1.3em]alig.west) -- (alig.west);
    \draw[->,line width=1.8pt,ublue] (alig.east) -- ([xshift=1.3em]alig.east);

    %%%%%%%%%%%%%%%%%% 4
    \node[prob,minimum width=0.5em] (rep31) at ([yshift=0em,xshift=2.5em]rep21.east) {};
    \node[prob,minimum width=1em] (rep32) at ([yshift=0.4em,xshift=0.15em]rep31.north) {};
    \node[](dot31) at ([yshift=0.4em,xshift=-0.2em]rep32.north) {.};
    \node[](dot32) at ([yshift=-0.05cm]dot31.north) {.};
    \node[](dot33) at ([yshift=-0.05cm]dot32.north) {.};
    \node[prob,minimum width=2.5em] (rep33) at ([yshift=1.6em,xshift=0.75em]rep32.north) {};

    %%%%%%%%%%%%%%%%% 5
    \node[representStyle,minimum width=1em,fill=orange!30] (rep42) at ([yshift=0.5em,xshift=5em]rep32.east) {};

    \draw[-,line width=1.8pt,ublue] ([xshift=2.6em,yshift=0.7em]rep32.east) -- ([xshift=3.5em,yshift=0.7em]rep32.east);
    \draw[-,line width=1.8pt,ublue] ([xshift=2.6em,yshift=0.25em]rep32.east) -- ([xshift=3.5em,yshift=0.25em]rep32.east);


    \node[minimum height=1em,inner sep=2pt,rounded corners=3pt,draw,fill=blue!20,anchor=west] (layerNorm) at ([xshift=-4.5em,yshift=-4em]alig.north) {\small Layer Norm};
    \node[minimum height=1em,inner sep=2pt,rounded corners=1pt,draw,fill=orange!20,shape=trapezium,trapezium stretches,trapezium angle=85,anchor=west] (conv) at ([xshift=1em]layerNorm.east) {\small Conv1D};
    \node[minimum height=1em,inner sep=2pt,rounded corners=3pt,draw,fill=green!20,anchor=west] (batchNorm) at ([xshift=1em]conv.east) {\small Batch Norm};
    \node[minimum height=1em,inner sep=2pt,rounded corners=3pt,draw,fill=red!20,anchor=west] (relu) at ([xshift=1em]batchNorm.east) {\small ReLU};

    \draw[->,ublue,line width=1pt]([xshift=-0.8em]layerNorm.west)--(layerNorm.west);
    \draw[->,ublue,line width=1.2pt](layerNorm.east)--(conv.west);
    \draw[->,ublue,line width=1.2pt](conv.east)--(batchNorm.west);
    \draw[->,ublue,line width=1.2pt](batchNorm.east)--(relu.west);
    \draw[->,ublue,line width=1.2pt](relu.east)--([xshift=0.8em]relu.east);

    \begin{pgfonlayer}{background}
      \node [rectangle,rounded corners=2pt,dashed,line width=1.5pt,minimum width=18em,minimum height=2em,draw=black!60,drop shadow,fill=gray!10] [fit = (layerNorm) (relu)] (box1) {};
      \draw[->,line width=1pt,dashed] (alig.south) -- ([xshift=-4.25em]box1.north);
    \end{pgfonlayer}
  
  %%%%%%%%% 图注

  \node[representStyle,minimum width=1em] (tuzhu1) at ([yshift=1.5em,xshift=-0.5em]rep3.north) {};
  \node[] (tuzhu11) at ([xshift=2.4em,yshift=0.35em]tuzhu1.east) {\footnotesize Multi-level};
  \node[] (tuzhu12) at ([xshift=3em,yshift=-0.4em]tuzhu1.east) {\footnotesize Representation};

  \node[prob,minimum width=1em] (tuzhu2) at ([yshift=0em,xshift=7em]tuzhu1.east) {};
  \node[] (tuzhu22) at ([xshift=1.6em]tuzhu2.east) {\footnotesize Weight};

  \node[representStyle,minimum width=1em,fill=orange!30] (tuzhu3) at ([yshift=0em,xshift=4.5em]tuzhu2.east) {};
  \node[] (tuzhu33) at ([xshift=1.6em,yshift=0.35em]tuzhu3.east) {\footnotesize Fusion};
  \node[] (tuzhu333) at ([xshift=3em,yshift=-0.4em]tuzhu3.east) {\footnotesize Representation};


  \node[](tmp)at ([xshift=0.3em]tuzhu1.west) {};
  \node[](tmp2)at ([xshift=-0.6em]tuzhu333.east) {};
  \node[](tmp3)at ([yshift=-0.8em]tuzhu11.north) {};
  \node[](tmp4)at ([yshift=0.8em]tuzhu12.south) {};

  \begin{pgfonlayer}{background}
    \node [rectangle,rounded corners=2pt,dashed,line width=1.5pt,minimum width=10em,draw=black!60,fill=white] [fit = (tmp) (tmp2) (tmp3) (tmp4)] (box1) {};
  \end{pgfonlayer}

  \end{tikzpicture}
\caption{The representation fusion method. It aligns multi-level representations to the same shapes then combines them.}
\label{alignment}
\end{figure}

==> fig/PDS.tex <==
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{fit,backgrounds}
\definecolor{ugreen}{rgb}{0,0.5,0}
\definecolor{myblue}{RGB}{30,144,255}
\usetikzlibrary{shadows}
\newlength{\heightSpan}
\begin{figure*}[t!]
  \centering
  \begin{tikzpicture}[scale=0.85]
    \tikzstyle{every node}=[scale=0.85]
    \setlength{\heightSpan}{1.5em}
    \tikzstyle{encoderStyle} = [minimum width=7em,inner sep=2pt,rounded corners=1pt,draw,fill=green!20]
    \tikzstyle{downModuleStyle} = [minimum width=7em,inner sep=2pt,rounded corners=1pt,draw,fill=red!15,shape=trapezium,trapezium stretches,trapezium angle=85]
    \tikzstyle{cellStyle} = [minimum height=1em,inner sep=2pt,rounded corners=1pt,draw,fill=teal!20,minimum width=1em]
    \tikzstyle{textBox} = []
    \tikzstyle{convStyle} = [minimum width=4em,inner sep=2pt,rounded corners=1pt,draw,fill=gray!10]
    \tikzstyle{prob} = [rectangle,fill=ugreen!40,minimum height=1em,anchor=west]
%%%% Speech Input
    \node[downModuleStyle] (down1) at (0,0) {Down-sampling};
    \node[encoderStyle] (encoder1) at ([yshift=\heightSpan]down1.north) {Encoder layers};
    \node[cellStyle,minimum width=7em] (cell1) at ([yshift=-\heightSpan]down1.south) {};
  
    \node[cellStyle,minimum width=5em] (cell2) at ([yshift=\heightSpan]encoder1.north) {};
    \node[downModuleStyle] (down2) at ([yshift=\heightSpan]cell2.north) {Down-sampling};
    \node[encoderStyle] (encoder2) at ([yshift=\heightSpan]down2.north) {Encoder layers};

    \node[cellStyle,minimum width=3.5em] (cell3) at ([yshift=\heightSpan]encoder2.north) {};
    \node[downModuleStyle] (down3) at ([yshift=\heightSpan]cell3.north) {Down-sampling};
    \node[encoderStyle] (encoder3) at ([yshift=\heightSpan]down3.north) {Encoder layers};

    \node[cellStyle,minimum width=2em] (cell4) at ([yshift=\heightSpan]encoder3.north) {};
    \node[downModuleStyle] (down4) at ([yshift=\heightSpan]cell4.north) {Down-sampling};
    \node[encoderStyle] (encoder4) at ([yshift=\heightSpan]down4.north) {Encoder layers};

    \node[cellStyle,minimum width=1.1em,minimum height=1.1em] (cell5) at ([yshift=\heightSpan]encoder4.north) {};
    \node[textBox] (speechInput) at ([yshift=-\heightSpan]cell1.south) {Speech Features};

    \begin{pgfonlayer}{background}
      \node [rectangle,rounded corners=2pt,dotted,line width=2pt,minimum width=8em,minimum height=4.2em,fill=cyan!5,draw=black!40] [fit = (down1) (encoder1)] (box1) {};
      \node [rectangle,rounded corners=2pt,dotted,line width=2pt,minimum width=8em,minimum height=4.2em,fill=cyan!5,draw=black!40] [fit = (down2) (encoder2)] (box2) {};
      \node [rectangle,rounded corners=2pt,dotted,line width=2pt,minimum width=8em,minimum height=4.2em,fill=cyan!5,draw=black!40] [fit = (down3) (encoder3)] (box3) {};
      \node [rectangle,rounded corners=2pt,dotted,line width=2pt,minimum width=8em,minimum height=4.2em,fill=cyan!5,draw=black!40] [fit = (down4) (encoder4)] (box4) {};
    \end{pgfonlayer}

    \draw[->] (cell1.north) -- (down1.south);
    \draw[->] (down1.north) -- (encoder1.south);
    \draw[->] (encoder1.north) -- (cell2.south);

    \draw[->] (cell2.north) -- (down2.south);
    \draw[->] (down2.north) -- (encoder2.south);
    \draw[->] (encoder2.north) -- (cell3.south);

    \draw[->] (cell3.north) -- (down3.south);
    \draw[->] (down3.north) -- (encoder3.south);
    \draw[->] (encoder3.north) -- (cell4.south);

    \draw[->] (cell4.north) -- (down4.south);
    \draw[->] (down4.north) -- (encoder4.south);
    \draw[->] (encoder4.north) -- (cell5.south);

%%%%最左边新增模块
    \node[downModuleStyle] (newDown1) at ([xshift=-11.5em]down1.west) {Down-sampling};
    \node[cellStyle,minimum width=7em] (newcell1) at ([yshift=-\heightSpan]newDown1.south){};
    \node[cellStyle,minimum width=5em] (newcell2) at ([yshift=\heightSpan]newDown1.north){};
    \node[downModuleStyle] (newDown2) at ([yshift=\heightSpan]newcell2.north) {Down-sampling};
    \node[cellStyle,minimum width=3.5em] (newcell3) at ([yshift=\heightSpan]newDown2.north){};
    \node[circle,minimum size=1.5em,draw,fill=yellow!20] (newcir) at ([yshift=1.3*\heightSpan]newcell3.north) {};
    \node[encoderStyle] (newEncoder) at ([yshift=\heightSpan]newcir.north){Encoder layers};
    \node[cellStyle,minimum width=3.5em] (newcell4) at ([yshift=\heightSpan]newEncoder.north){};
    \node[textBox] (newPe) at ([xshift=3em]newcir.east) {PE};
    \node[textBox] (newSpeech) at ([yshift=-\heightSpan]newcell1.south) {Speech Features};
    % \draw[->](newSpeech.north)--(newcell1.south);
    \draw[->](newcell1.north)--(newDown1.south);
    \draw[->](newDown1.north)--(newcell2.south);
    \draw[->](newcell2.north)--(newDown2.south);
    \draw[->](newDown2.north)--(newcell3.south);
    \draw[->](newcell3.north)--(newcir.south);
    \draw[->](newcir.north)--(newEncoder.south);
    \draw[->](newEncoder.north)--(newcell4.south);
    \draw[->](newPe.west)--(newcir.east);
    \draw[-](newcir.west)--(newcir.east);
    \draw[-](newcir.north)--(newcir.south);


%%%% Fusion module
    \node[convStyle,minimum height=1.1em] (conv1) at ([xshift=9em]cell5.east) {\small Alignment};
    \node[convStyle,minimum height=1.1em] (conv2) at ([yshift=-0.7em]conv1.south) {\small Alignment};
    \node[convStyle,minimum height=1.1em] (conv3) at ([yshift=-0.7em]conv2.south) {\small Alignment};
    \node[convStyle,minimum height=1.1em] (conv4) at ([yshift=-0.7em]conv3.south) {\small Alignment};

    \node[cellStyle,minimum height=1.1em,minimum width=1.1em,fill=myblue!30] (c11) at ([xshift=2em]conv1.east){};
    \node[cellStyle,minimum height=1.1em,minimum width=1.1em,fill=myblue!30] (c12) at ([yshift=-0.7em]c11.south){};
    \node[cellStyle,minimum height=1.1em,minimum width=1.1em,fill=myblue!30] (c13) at ([yshift=-0.7em]c12.south){};
    \node[cellStyle,minimum height=1.1em,minimum width=1.1em,fill=myblue!30] (c14) at ([yshift=-0.7em]c13.south){};
    \node[prob,minimum height=1.1em,minimum width=0.7cm] (c21) at ([xshift=2.2em]c11.east){};
    \node[prob,minimum height=1.1em,minimum width=0.5cm] (c22) at ([xshift=2.2em]c12.east){};  
    \node[prob,minimum height=1.1em,minimum width=0.3cm] (c23) at ([xshift=2.2em]c13.east){};
    \node[prob,minimum height=1.1em,minimum width=0.1cm] (c24) at ([xshift=2.2em]c14.east){};
    \node[cellStyle,minimum height=1.1em,minimum width=1.1em,fill=myblue!30] (c31) at ([xshift=3.8em,yshift=-0.3em]c22.south){};
    \node[textBox](featureWeight) at ([xshift=1.0em,yshift=-1em]c14.south) {\small Representation Weight};
    \node[] (tmp) at ([yshift=-0.0em]featureWeight.north) {};

    \begin{pgfonlayer}{background}
      \node [rectangle,rounded corners=2pt,dotted,line width=2pt,minimum width=14.5em,minimum height=8em,fill=cyan!5,draw=black!40] [fit = (c11) (c31) (tmp) (conv1)] (box5) {};
    \end{pgfonlayer}

    \node[textBox](fusion) at ([yshift=-1.3em]box5.south) {Representation Fusion};

    \draw[->] (conv1.east) -- (c11.west);
    \draw[->] (conv2.east) -- (c12.west);
    \draw[->] (conv3.east) -- (c13.west);
    \draw[->] (conv4.east) -- (c14.west);

    % 乘号
    % myblue!60
    \draw [-,black!70,line width=2pt] ([xshift=0.5em]c12.east) -- ([xshift=1.7em]c13.east);
    \draw [-,black!70,line width=2pt] ([xshift=0.5em]c13.east) -- ([xshift=2.8em]c12.west);
    %等号
    \draw [-,black!70,line width=2pt] ([xshift=1.2em]c22.south) -- ([xshift=2.5em]c22.south);
    \draw [-,black!70,line width=2pt] ([xshift=1.2em,yshift=-0.5em]c22.south) -- ([xshift=2.5em,yshift=-0.5em]c22.south);
    %大箭头
    \draw[->,line width=2pt,black!70]([xshift=1em]c31.east)--([xshift=2.5em]c31.east);

    %圆角线
    \draw[->,rounded corners=3pt] (cell2.east) -- +(3.0em,0) |- (conv4.west);
    \draw[->,rounded corners=3pt] (cell3.east) -- +(3.2em,0) |- (conv3.west);
    \draw[->,rounded corners=3pt] (cell4.east) -- +(3.4em,0) |- (conv2.west);
    \draw[->,rounded corners=3pt] (cell5.east) -- (conv1.west);

%%% Down-sampling module
    \node[](t1) at ([xshift=13em,yshift=1em]cell1.east){};
    \node[](t2) at ([yshift=8em]t1.north){};
    %\node [rectangle,rounded corners=2pt,dotted,line width=2pt,minimum width=10em,minimum height=4em,draw=black!40,fill=cyan!5] [fit = (t1)(t2)] (box6) {};

    \node[cellStyle,minimum width=7em] (downCell) at ([xshift=13em]cell1.east) {};
    \node[textBox](downSampling) at ([yshift=-\heightSpan]downCell.south){Down-sampling};
    \node[minimum width=7em,inner sep=4pt,rounded corners=1pt,draw,fill=orange!20,shape=trapezium,trapezium stretches,trapezium angle=85] (downConv) at ([yshift=2em]downCell.north){Conv1D};
    \node[minimum width=7em,inner sep=4pt,rounded corners=1pt,draw,fill=blue!20] (layerNorm) at ([yshift=2em]downConv.north) {Layer Norm};
    \node[circle,minimum size=1.5em,draw,fill=yellow!20] (cir) at ([yshift=2em]layerNorm.north) {};
    \node[textBox] (pe) at ([xshift=3em]cir.east) {PE};
    \node[cellStyle,minimum width=5em](downCell2) at ([yshift=\heightSpan]cir.north) {};

    \begin{pgfonlayer}{background}
      \node[rectangle,rounded corners=2pt,draw=black,minimum width=13em,minimum height=13em,drop shadow,fill=gray!10,dotted,line width=2pt,draw=black!40][fit = (downCell2) (downCell)] (box6-2) {};
    \end{pgfonlayer}
    \draw[-,dotted,line width=2pt,draw=black!40](down1.east)--([yshift=6.5em]box6-2.west);
    \draw[-,dotted,line width=2pt,draw=black!40](down1.east)--([yshift=-6.5em]box6-2.west);

    \draw[-](cir.west)--(cir.east);
    \draw[-](cir.north)--(cir.south);
    \draw[->](downCell.north)--(downConv.south);
    \draw[->](downConv.north)--(layerNorm.south);
    \draw[->](layerNorm.north)--(cir.south);

    \draw[->](pe.west)--(cir.east);
    \draw[->](cir.north)--(downCell2.south);

    %%%% sub caption
    \node[textBox] (a) at ([yshift=-1em]newSpeech.south){\normalsize (a) Stack};
    \node[textBox] (b) at ([yshift=-1em,xshift=8em]speechInput.south){\normalsize (b) PDS};

    %%%%% 公式
    \node[textBox](formula1)at([xshift=-3.5em]cell1.west){$H_0$:$T \times D_0$};
    \draw[-,dotted,line width=1pt](formula1.east)--([xshift=-0.5em]cell1.west);
    \node[textBox](formula2)at([xshift=-4.5em]cell2.west){$H_1$:$\frac{T}{2} \times D_1$};
    \draw[-,dotted,line width=1pt](formula2.east)--([xshift=-0.5em]cell2.west);
    \node[textBox](formula3)at([xshift=-5.25em]cell3.west){$H_2$:$\frac{T}{4} \times D_2$};
    \draw[-,dotted,line width=1pt](formula3.east)--([xshift=-0.5em]cell3.west);
    \node[textBox](formula4)at([xshift=-6.0em]cell4.west){$H_3$:$\frac{T}{8} \times D_3$};
    \draw[-,dotted,line width=1pt](formula4.east)--([xshift=-0.5em]cell4.west);
    \node[textBox](formula5)at([xshift=-6.45em]cell5.west){$H_4$:$\frac{T}{16} \times D_4$};
    \draw[-,dotted,line width=1pt](formula5.east)--([xshift=-0.5em]cell5.west);
    %最左边那一列
    \node[textBox](formula11)at([xshift=-3.5em]newcell1.west){$H_0$:$T\times D_0$};
    \draw[-,dotted,line width=1pt](formula11.east)--([xshift=-0.5em]newcell1.west);
    \node[textBox](formula12)at([xshift=-4.5em]newcell2.west){$H_1$:$\frac{T}{2} \times D$};
    \draw[-,dotted,line width=1pt](formula12.east)--([xshift=-0.5em]newcell2.west);
    \node[textBox](formula13)at([xshift=-5.25em]newcell3.west){$H_2$:$\frac{T}{4} \times D$};
    \draw[-,dotted,line width=1pt](formula13.east)--([xshift=-0.5em]newcell3.west);
    \node[textBox](formula14)at([xshift=-5.25em]newcell4.west){$H_L$:$\frac{T}{4} \times D$};
    \draw[-,dotted,line width=1pt](formula14.east)--([xshift=-0.5em]newcell4.west);

  \end{tikzpicture}
  \caption{Comparison of the Stack and PDS methods. $T$ and $D_0$ represent the length and dimension of the input speech features respectively. In PDS, the length of speech features are condensed to $T/16$ progressively. }
  \label{pds}
\end{figure*}

